QCL active region overheat in pulsed mode: effects of non-equilibrium heat dissipation on laser performance

Quantum cascade lasers are of high interest in the scientific community due to unique applications utilizing the emission in mid-IR range. The possible designs of QCL are quite limited and require careful engineering to overcome some crucial disadvantages. One of them is an active region (ARn) overheat, that significantly affects the laser characteristics in the pulsed operation mode. In this work we consider the effects related to the non-equilibrium temperature distribution, when thermal resistance formalism is irrelevant. We employ the heat equation and discuss the possible limitations and structural features stemming from the chemical composition of the AR. We show that the presence of alloys in the ARn structure fundamentally limits the heat dissipation in pulsed and CW regimes due to their low thermal conductivity. Also the QCL post-growths affects the thermal properties of a device only in (near)CW mode while it is absolutely invaluable in the pulsed mode

==> trash.tex <==


\clearpage
\newpage



\begin{figure}
\includegraphics[scale=0.31]{slope.pdf}
\caption{Experimental curve of the laser emission under different pump. Dashed line is fitted in the very beginning of the pulse to depict the moment of crossing X-axis where by definition the threshold current increases up to pump current due to heating of the active region}
\label{fig-slope}
\end{figure}

The temperature dependence of the threshold current\cite{fehse02} can be treated with the well-known expression\cite{}:

\begin{equation}
    I_{thr}=I^{RT}_{thr} e^{\frac{k(T-RT)}{\hbar \omega_0}} =I^{RT}_{thr} e^{\frac{\Delta T}{\hbar \omega_0}} ,
    \label{eq:ithrtempdep}
\end{equation}

\noindent \textcolor{red}{describe hw0 in detail} where $I_{thr}$ is an instantaneous threshold current at specified instantaneous temperature T of an active region, $I^{RT}_{thr}$ is a threshold current when an active region is at room temperature (RT), $\hbar \omega_0$ - is a probability (power) of a non-radiative relaxation rate per effective phonon mode specified in term of energy (constant in the temperature range of interest).


In the formula above there are three unknown values: instantaneous temperature of active region, the value of threshold current at room temperature and effective phonon mode energy. %Assuming the value of QCL heat capacity about $C_{QCL}$=2.25$\cdot$10$^{-7}$~J~K$^{-1}$\cite{}, pump voltage of $U_{exp}$ of 10~V, we tune the value of $\hbar \omega_0$ to achieve the self-consistent estimation of the threshold current.
We will obtain the first value by means of one dimensional heat equation treated with the model described below. We assume that the active region, the upper cladding and the substrate are made of compound with thermal properties of InP. We assume that there is an infinite environment of air (which convection is disabled) above the upper cladding. We consider the substrate coupled to the infinite slab of copper, which temperature (at infinity) equals to room temperature. The thicknesses of finite layers are 2, 5 and 5~$\mu$m correspondingly.

\begin{figure}
\includegraphics[scale=0.31]{heatmap.pdf}
\caption{heatmap of QCL under 500~ns pump pulse}
\label{fig-heatmap}
\end{figure}

Heating profile for the active region for pump currents equal to 4.5~A, 5.6~A and 6.8~A are depicted in Fig.~\ref{fig-ARheat}.

\begin{figure}
\includegraphics[scale=0.31]{ARheat.pdf}
\caption{temperature profile of an active region of QCL.}
\label{fig-ARheat}
\end{figure}



\begin{table}
\caption{Experimental data allowing extraction of the self-consistent pair of $I^{RT}_{thr}$ and $\hbar \omega_0$, with the latter equal to 60~meV}
\begin{tabular}{|m{1.5cm}|m{1.5cm}|m{1cm}|m{3cm}|} \hline
$I_{pump}$, A & modelled $T_{AR}$ after 100~ns, K $\Delta t$, ns & Tcutoff, ns & expected temperature according first 100 ns \\ \hline \hline
4.5 & XXX  & 400  &  \\
5.6 & YYY  & 800  &  \\
6.8 & ZZZ  & 1200 &  \\ \hline
\end{tabular}
\label{tbl:ithrestimation}
\end{table}

Here we obtain the value of the threshold current specified for room temperature via tuning of the $\hbar \omega_0$. Averaging over the last column we assess the value of threshold current as $I^{RT}_{thr}$=4.13~A.

With the value of threshold current at room temperature on hands one can assess the behaviour of the light-current characteristic of the device for varying temperatures via eq.~(\ref{eq:ithrtempdep}). Consider the L-I curve typical for RT, 350~K, and 400~K (see Fig.~\ref{fig-collection}). These function have the threshold currents of 4.13~A, 4.42~A, and 4.74~A correspondingly. The decrease of L-I curve slope is obtained from the scratch.

\begin{figure}
\includegraphics[scale=0.31]{licollection.pdf}
\caption{Light-Current characteristics of a device modeled at different temperatures of active region. Colored arrows show degradation path of a light pulse depicted in Fig.~\ref{fig-slope}. Intensity of a signal after 500~ns strongly suggests high temperature (about 100~K) of a device in the end of the pump interval}
\label{fig-collection}
\end{figure}

If one assumes that the decrease of a light pulse is governed by the heating, then it is straightforwardly follows from Fig.~\ref{fig-collection} that the heating of the active region to the end of 500~ns pump pulse is in the order of 100~K. Thus heating of active region during 30~ns  time interval is about 6~K.



